Disaggregating Non-Volatile Memory for Throughput-Oriented Genomics Workloads

Massive exploitation of next-generation sequencing technologies requires dealing with both: huge amounts of data and complex bioinformatics pipelines. Computing architectures have evolved to deal with these problems, enabling approaches that were unfeasible years ago: accelerators and Non-Volatile Memories (NVM) are becoming widely used to enhance the most demanding workloads. However, bioinformatics workloads are usually part of bigger pipelines with different and dynamic needs in terms of resources. The introduction of Software Defined Infrastructures (SDI) for data centers provides roots to dramatically increase the efficiency in the management of infrastructures. SDI enables new ways to structure hardware resources through disaggregation, and provides new hardware composability and sharing mechanisms to deploy workloads in more flexible ways. In this paper we study a state-of-the-art genomics application, SMUFIN, aiming to address the challenges of future HPC facilities.

==> resourcesharing.tex <==
\section{Experiment 1. Resource sharing}
As stated before, SDI will switch the paradigm from single-workload resource usage to resource sharing. To explore the impact of sharing on workloads' performance we have partitioned our NVMe cards, and on every partition we run a workload instance. Running concurrently as many instances as partitions (each instance runs on its own partition) provides the resource sharing. In a real SDI environment each partition would be seen for the instances as a single storage unit, hiding what is behind. 









%\begin{figure*}%
%	\centering
%	\subfloat[1x NVMeOF]{\includegraphics[width=0.98\columnwidth]{images/fio_nvme01_usage_boxplot.pdf}}\qquad
%	\subfloat[2x NVMeOF]{\includegraphics[width=0.98\columnwidth]{images/fio_raid0_nvme01-02_usage_boxplot.pdf}}\qquad
%	\caption{FIO. Write Bandwidth - Sequential}
%	\label{fig:fio-bandwidth}
%\end{figure*}





%\begin{figure}%
%	\centering
%	\subfloat[1x NVMe]{\includegraphics[width=0.98\columnwidth]{images/3sim-1xnvme/iostat-nvm01.png}}\qquad
%	\subfloat[2xNVMe]{\includegraphics[width=0.98\columnwidth]{images/3sim-2xnvme/iostat-nvm01.png}}\qquad
%	\caption{Bandwidth as measured in the Flash Pool server - 3x instances of Smufin for 1x or 2x NVMe}
%	\label{fig:a}
%\end{figure}



















\subsection{Composed memory}
\label{subsec:composedmemory}

